ICLR: In-Context Learning of Representations

Recent work has demonstrated that semantics specified by pretraining data influence how representations of different concepts are organized in a large language model (LLM). However, given the open-ended nature of LLMs, e.g., their ability to in-context learn, we can ask whether models alter these pretraining semantics to adopt alternative, context-specified ones. Specifically, if we provide in-context exemplars wherein a concept plays a different role than what the pretraining data suggests, do models reorganize their representations in accordance with these novel semantics? To answer this question, we take inspiration from the theory of conceptual role semantics and define a toy "graph tracing" task wherein the nodes of the graph are referenced via concepts seen during training (e.g., apple, bird, etc.) and the connectivity of the graph is defined via some predefined structure (e.g., a square grid). Given exemplars that indicate traces of random walks on the graph, we analyze intermediate representations of the model and find that as the amount of context is scaled, there is a sudden re-organization from pretrained semantic representations to in-context representations aligned with the graph structure. Further, we find that when reference concepts have correlations in their semantics (e.g., Monday, Tuesday, etc.), the context-specified graph structure is still present in the representations, but is unable to dominate the pretrained structure. To explain these results, we analogize our task to energy minimization for a predefined graph topology, providing evidence towards an implicit optimization process to infer context-specified semantics. Overall, our findings indicate scaling context-size can flexibly re-organize model representations, possibly unlocking novel capabilities.

==> deprecated_material.tex <==
Neural networks can demonstrate sudden changes in behavior, often referred to as \emph{emergence}, when scaled in terms of model parameters or training data.
Such discontinuous behavior can lead to unforeseen effects, raising a concern for safe development of AI systems and calling for a scientific understanding of said phenomena.
A relatively understudied dimension of scale with regards to emergent behavior is inference-time budget.
We study this relationship using synthetic in-context world modeling tasks, in which we demonstrate that networks abruptly solve novel tasks given sufficient exemplars during inference.
We further find geometric representations in the network's activations that reflect the structure of the in-context data, around the same time at which the model starts to make valid predictions.
We provide analytical predictions for when such transition points of in-context emergence can be expected, as a function of task complexity.
Finally we empirically verify our predictions, demonstrating that our theorems hold in practice.
Overall, we demonstrate an analytical framework to characterize and predict in-context emergence in neural networks.



% Representation learning has been central to deep learning's evolution. While interpretable structures have been observed in pre-trained models' representations, an important question arises: Do networks develop such interpretable structures during in-context learning? Using synthetic sequence data derived from underlying geometrically structured graphs (e.g., grids, rings), we provide affirmative evidence that language models develop internal representations mirroring these geometric structures during in-context learning. Furthermore, we demonstrate how in-context examples can override semantic priors by constructing a representation in dimensions other than the one used by the prior.
% Overall, our study demonstrates that models can form meaningful representations solely from in-context exemplars.


% Neural networks can demonstrate sudden changes in behavior, often referred to as \emph{emergence}, when scaled in terms of model parameters or training data.



% Such discontinuous behavior can lead to unforeseen effects, raising a concern for safe development of AI systems and calling for a scientific understanding of said phenomena.
% A relatively understudied dimension of scale with regards to emergent behavior is inference-time budget.
% We study this relationship using synthetic in-context world modeling tasks, in which we demonstrate that networks abruptly solve novel tasks given sufficient exemplars during inference.
% We further find geometric representations in the network's activations that reflect the structure of the in-context data, around the same time at which the model starts to make valid predictions.
% We provide analytical predictions for when such transition points of in-context emergence can be expected, as a function of task complexity.
% Finally we empirically verify our predictions, demonstrating that our theorems hold in practice.
% Overall, we demonstrate an analytical framework to characterize and predict in-context emergence in neural networks.
% \\
% %H: Hello. I actually like what you are writing! do you want to take a lead? haha
% %C: I'm stuck.  can you next token generate?
% %H: will try
% %C: I'm giving the baton to Ekdeep and Hidenori and will go generate markov figures
% Recent efforts to extract the most out of a pretrained language model has lead to a new frontier: inference scaling. While many empirical studies investigates the performance aspect of inference scaling, the fundamental principles driving the performance are not yet understood. In this study, we investigate into two specific questions: 1) Do models form a novel task specific representations solely from in-context exemplars? 2) Do the structures of representations 
% 2) Is there a mechanism explaining the non linear increase, i.e. emergence, of in context performance? We define a graph of tokens with \emph{no} semantic geometry aligned with the graph topology.



\iffalse
\clearpage 


Neural networks behave differently when scaled in certain dimensions, such as the size of model parameters or learning data (TODO).
Interestingly, as networks scale, some changes in behaviors seem to appear abruptly.
Such discontinuity, often referred to as \textbf{emergence} or \textbf{phase transitions}, can lead to substantial improvements for downstream tasks.
However, it can also lead to unforeseen effects (TODO), raising a concern for safe development of AI systems.
This motivates the need for a scientific understanding of the causal relationship between scaling and emergence.

Such a relationship has been studied before (TODO).
However, most prior work studies scaling dimensions with respect to model parameters or training data (TODO).
A relatively understudied dimension of scale is inference budget.
Namely, auto-regressive models such as transformers can execute more computations with longer input contexts, given the larger number of activations that naturally arise.
This is often attributed to the success of paradigms like chain-of-thought reasoning or recent popular models like OpenAI-o1 (TODO).
As inference budget is scaled, perhaps most surprising is the model's ability to solve novel tasks that are specified solely by inference-time exemplars, often referred to as in-context learning (ICL; TODO-cite).
Though the relationship between ICL and the scale of model parameter size or training data has been studied before (TODO), its relationship with scaling inference budget has been understudied.
In this work, we aim to fill this gap.

To this point, we ask: \textbf{Does emergence occur in-context as well? If so, can we predict and characterize when to expect emergence?}

To study our question, we formulate in-context world modeling tasks, in which we design an underlying ``world'' that must be learned before a model is able to make valid predictions.
Such tasks are suitable for our study in that the model's performance should scale with the number of observations (i.e., context size) that it sees.

Similar to observations seen in other regimes of scaling, we observe a similar discontinuous increase in the model's in-context task performance as we scale our context length.
In addition, to the first of our knowledge, we find geometric representations of the underlying ``world'' in the activations of our model around the same time at which the model learns the task (Section~\ref{sec:uncovering_in_context_task_representations}).

Given such observations, we draw inspiration from spectral graph theory and studies of percolation phase transitions from physics (TODO) to make predictive claims regarding in-context emergence.
Namely, we characterize the model's learning of the task as an \emph{energy minimization process} in search of the correct structural representation of the data.
This allows us to make analytical predictions for transition points at which we can expect emergent behavior, as a function of task complexity (Section~\ref{sec:theory}).

Finally, we verify our analytical predictions with a range of empirical experiments, in which we control for task complexity.

In summary, our contributions are as follows.

\begin{itemize}
  \item \textbf{Concurrent emergence of in-context abilities and geometric task representations.}
    In Section~\ref{sec:uncovering_in_context_task_representations} we demonstrate emergent behavior for in-context world modeling tasks, and that geometric representations of the data appear concurrently in the activations of the model once the model learns the task.
  
  \item \textbf{Predicting transition points for in-context emergence.}
    In Section~\ref{sec:theory} we provide theorems to predict the transition point in which in-context emergent behavior is expected as a function of task complexity.
    
  \item \textbf{Empirical verification of transition point predictions.}
    Lastly, in Section~\ref{sec:verifying_theory} we verify our theorems with empirical experiments, demonstrating that our theorems hold in practice.
\end{itemize}
\fi


==> intro2.tex <==
Modern large language models (LLMs) can learn a wide range of capabilities from pre-training.
Interestingly, a growing line of work demonstrates that pre-trained LLMs can form interpretable geometric representations that reflect structured patterns found in its training data.
For instance, \cite{li2022emergent} deploys synthetic data to demonstrate that LLMs can form \emph{world representations} that mirror the underlying data-generating process, while \cite{engels2024languagemodelfeatureslinear} shows that periodic concepts such as days of the week are represented as a ring topology.
%C
% As do we see analogous phenomena in ICL?
Meanwhile, prior work suggests that said capabilities of pre-trained LLMs often appear ``abruptly'' -- a discontinuous phenomenon we often refer to as ``emergence'' -- as models are scaled up in the size of data, model parameters, or compute resources.
However, a relatively easier dimension to scale is inference-time compute, which may attribute to the success of paradigms like chain-of-thought or recent models like o1.

This raises a series of fundamental questions:
Can novel capabilities also emerge from scaling inference budget?
If so, do models dynamically develop context-specific representations?
What are the causal factors driving such inference-time emergent capabilities?
Beyond advancing our scientific understanding, identifying such causal factors is crucial for managing risks associated with deploying large-scale AI systems.

To study these questions, we use \emph{in-context learning} (ICL).
Specifically, we introduce a toy graph navigation task, where we ``spatially'' organize a set of randomly selected words on structured graphs (e.g., grids and rings) without any reflection to the words' semantic meanings.
We then generate sequences of tokens following traces of random walks on the graph as in-context inputs to the model, and evaluate whether the model's next token predictions adhere to the graph topology underlying the data generating process.

In this setup, we find,
\begin{enumerate}
    \item \textbf{Emergence of in-context abilities:} As the number of context exemplars increases, the model's capability to navigate the graph's topology suddenly emerges.
    \item \textbf{Emergence of structured task representations in-context:} Around the same time at which the model's capability emerges, we also see an emergent reorganization of representations mirroring the graph topology underlying the data-generating process.
    \item \textbf{Percolation theory predicts transition points for in-context emergence:} Inspired by percolation transition in complex systems, we theoretically derive a prediction for the transition point of emergent in-context ability, which we verify empirically.
\end{enumerate}

